Deep Learning and Data Assimilation for Real-Time Production Prediction in Natural Gas Wells

The prediction of the gas production from mature gas wells, due to their complex end-of-life behavior, is challenging and crucial for operational decision making. In this paper, we apply a modified deep LSTM model for prediction of the gas flow rates in mature gas wells, including the uncertainties in input parameters. Additionally, due to changes in the system in time and in order to increase the accuracy and robustness of the prediction, the Ensemble Kalman Filter (EnKF) is used to update the flow rate predictions based on new observations. The developed approach was tested on the data from two mature gas production wells in which their production is highly dynamic and suffering from salt deposition. The results show that the flow predictions using the EnKF updated model leads to better Jeffreys' J-divergences than the predictions without the EnKF model updating scheme.

==> Results_discussion_old.tex <==
Before we get ahead of ourselves, let's check what the model produces. See if it follows a normal distribution. Figure~\ref{fig:histoplot_jul20_27} shows a typical histogram plot for the ensembles at a particular timestep.

\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{./Figures/plain_monte_carlo_jul20_jul27_histoplot}
\caption{Histogram plot of a typical time step with a Gaussian distribution overlay}
\label{fig:histoplot_jul20_27}
\end{figure}

Yes! Indeed it's normal distribution. We can use EnKF! Let's examine the time series for the plain monte carlo case to see how well our baseline model did.


\begin{figure}
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{./Figures/plain_monte_carlo_jul20_jul27}
        \caption{Timeseries Plot}
        \label{fig:Timeseries:base_jul20_27}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{./Figures/plain_monte_carlo_jul20_jul27_correlation_plot}
        \caption{Correlation Plot}
        \label{fig:Correlation:base_jul20_27}
    \end{subfigure}
    \caption{Predictions of baseline model for July 20-27, 2012 dataset}\label{fig:base_jul20_27}
\end{figure}

Results show that with the EnKF model updating scheme, for almost all the dataset ranges, the one timestep ahead prediction for the model improved compared to the baseline trained model.

\begin{figure}[h]
\centering
\includegraphics[width=0.45\textwidth]{./Figures/enkf_predicted_jul20_jul27}
\caption{Improved prediction for the model using the EnKF state update}
\label{fig:enkf_timeseries_jul20_27}
\end{figure}

Wow! Amazing! We improved the prediction from $R^2 = 0.67$ to $R^2 = 0.88$! Just like that! Let's see if the situation is improved for the other ranges in the datasets.

For the other dataset, let's do March 10-24, 2013. Let's see how it performs.
Baseline case already performs quite well for this dataset as we can see from Figure~\ref{fig:base_mar_2013}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{./Figures/plain_monte_carlo_mar_2013}
        \caption{Timeseries Plot}
        \label{fig:Timeseries:base_mar_2013}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{./Figures/plain_monte_carlo_mar_2013_correlation_plot}
        \caption{Correlation Plot}
        \label{fig:Correlation:base_mar_2013}
    \end{subfigure}
    \caption{Predictions of baseline model for July 20-27, 2012 dataset}\label{fig:base_mar_2013}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{./Figures/enkf_predicted_mar_2013}
        \caption{Timeseries Plot}
        \label{fig:Timeseries:enkf_mar_2013}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{./Figures/enkf_predicted_mar_2013_correlation_plot}
        \caption{Correlation Plot}
        \label{fig:Correlation:enkf_mar_2013}
    \end{subfigure}
    \caption{Predictions of baseline model for July 20-27, 2012 dataset}\label{fig:enkf_mar_2013}
\end{figure}

The EnKF update does seem to not do better, but the confidence interval has shrunk nearing the end which could indicate that the model is more confident of the predictions barring any fast dynamical transients (i.e. a few timesteps before and after well shutin)
